The Collimation and Energetics of the Brightest Swift Gamma-Ray Bursts

Long-duration gamma-ray bursts (GRBs) are widely believed to be highly-collimated explosions (opening angle theta ~ 1-10 deg). As a result of this beaming factor, the true energy release from a GRB is usually several orders of magnitude smaller than the observed isotropic value. Measuring this opening angle, typically inferred from an achromatic steepening in the afterglow light curve (a "jet" break), has proven exceedingly difficult in the Swift era. Here we undertake a study of five of the brightest (in terms of the isotropic prompt gamma-ray energy release, E(gamma, iso)) GRBs in the Swift era to search for jet breaks and hence constrain the collimation-corrected energy release. We present multi-wavelength (radio through X-ray) observations of GRBs 050820A, 060418, and 080319B, and construct afterglow models to extract the opening angle and beaming-corrected energy release for all three events. Together with results from previous analyses of GRBs 050904 and 070125, we find evidence for an achromatic jet break in all five events, strongly supporting the canonical picture of GRBs as collimated explosions. The most natural explanation for the lack of observed jet breaks from most Swift GRBs is therefore selection effects. However, the opening angles for the events in our sample are larger than would be expected if all GRBs had a canonical energy release of ~ 10e51 erg. The total energy release we measure for those "hyper-energetic" (E(total) >~ 10e52 erg) events in our sample is large enough to start challenging models with a magnetar as the compact central remnant.

==> tab1.tex <==
\ProvidesFile{060418rad.tab.tex}

\begin{deluxetable}{crrr}
  \tabletypesize{\scriptsize}
  \tablecaption{Radio Observations of GRB\,060418}
  \tablecolumns{4}
  \tablewidth{0pc}
  \tablehead{\colhead{UT Date\tablenotemark{a}} &
             \colhead{Time Since Burst\tablenotemark{b}} 
             & \colhead{Frequency} & \colhead{Flux Density\tablenotemark{c}} \\
             & \colhead{(d)} & \colhead{(GHz)} & \colhead{($\mu$Jy)}
            }
  \startdata
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  2006 Apr 19.50 & 1.37 & 8.46 & $105 \pm 45$ \\
  2006 Apr 22.43 & 4.30 & 8.46 & $148 \pm 44$ \\
  2006 Apr 25.42 & 7.29 & 8.46 & $242 \pm 59$ \\
  2006 Apr 27.25 & 9.12 & 8.46 & $113 \pm 43$ \\
  2006 May 4.15 & 16.02 & 8.46 & $184 \pm 39$ \\
  2006 May 6.20 & 18.07 & 8.46 & $158 \pm 31$ \\
  2006 May 9.17 & 21.04 & 8.46 & $< 84$ \\
  2006 May 11.17 & 23.04 & 8.46 & $136 \pm 36$ \\
  2006 Jun 8.21 & 51.08 & 8.46 & $< 78$ \\
  2006 Jun 25.27 & 68.14 & 8.46 & $< 62$ \\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \enddata
  \tablenotetext{a}{UT at midpoint of exposure.}
  \tablenotetext{b}{Time from mid-point of exposure to \Swift-BAT trigger.}
  \tablenotetext{c}{Upper limits are reported as 2$\sigma$ rms per beam area.}
\label{tab:060418rad}
\end{deluxetable}

%\end{input}


==> tab2.tex <==
\ProvidesFile{080319Brad.tab.tex}

\begin{deluxetable}{crrr}
  \tabletypesize{\scriptsize}
  \tablecaption{Radio/Sub-mm Observations of GRB\,080319B}
  \tablecolumns{4}
  \tablewidth{0pc}
  \tablehead{\colhead{UT Date\tablenotemark{a}} &
             \colhead{Time Since Burst\tablenotemark{b}} 
             & \colhead{Frequency} & \colhead{Flux Density\tablenotemark{c}} \\
             & \colhead{(d)} & \colhead{(GHz)} & \colhead{($\mu$Jy)}
            }
  \startdata
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  2008 Mar 20.48 & 1.11 & 95.0 & $< 500$ \\
  2008 Mar 21.56 & 2.30 & 4.86 & $204 \pm 40$ \\
  2008 Mar 21.56 & 2.30 & 8.46 & $232 \pm 42$ \\
  2008 Mar 21.81 & 2.55 & $1.90 \times 10^{4}$ & $35.7 \pm 3.9$ \\
  2008 Mar 26.48 & 7.22 & 4.86 & $167 \pm 61$ \\
  2008 Mar 26.48 & 7.22 & 8.46 & $< 110$ \\
  2008 Mar 29.89 & 10.63 & $1.90 \times 10^{4}$ & $< 8.0$ \\
  2008 Dec 25.83 & 281.57 & 1.46 & $< 28$ \\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \enddata
  \tablenotetext{a}{UT at midpoint of exposure.}
  \tablenotetext{b}{Time from mid-point of exposure to \Swift-BAT trigger.}
  \tablenotetext{c}{Upper limits are reported as 2$\sigma$ rms per beam area.}
\label{tab:080319Brad}
\end{deluxetable}

%\end{input}


==> tab3.tex <==
\ProvidesFile{050820Amodels.tab.tex}

\begin{deluxetable}{r|cccccccc}
  \tabletypesize{\scriptsize}
  \tablecaption{GRB\,050820A Forward Shock Best Fit Parameters}
  \tablecolumns{9}
  \tablewidth{0pc}
  \tablehead{\colhead{Medium Type\tablenotemark{a}} & 
             \colhead{$E_{\mathrm{KE,iso}}$} & \colhead{$n$} & 
             \colhead{$\epsilon_{e}$} & \colhead{$\epsilon_{B}$} & 
             \colhead{$\theta$} & \colhead{$p$} & \colhead{$A_{V}$(host)} & 
             \colhead{$\chi^{2}_{\mathrm{r}}$ (d.o.f.)} \\ 
             & \colhead{($10^{52}$\,erg)} & \colhead{(cm$^{-3}$)} &
             & \colhead{($\%$)} & \colhead{($^{\circ}$)} & & \colhead{(mag)} &
            }
  \startdata
  ISM-1 & $537_{-95}^{+80}$ & $0.18_{-0.07}^{+0.12}$ & $0.13 \pm 0.02$ & 
     $0.0022_{0.0004}^{+0.0011}$ & $6.6_{-0.3}^{+0.5}$ & $1.75 \pm 0.02$ &
     $0.11_{-0.02}^{+0.03}$ & 1.34 (76) \\
  ISM-2 & $410_{-25}^{+19}$ & $(3.9 \pm 1.0) \times 10^{-4}$ &
     $0.14_{-0.01}^{+0.02}$ & $1.3_{-0.1}^{+0.3}$ & $3.0 \pm 0.1$ & 
     $2.30_{-0.04}^{+0.03}$ & $< 0.049$\tablenotemark{b} & 1.31 (76) \\
  \enddata
  \tablenotetext{a}{Radial profile of the circumburst medium.  
    $\rho \propto r^{0}$ for an ISM-like medium; $\rho \propto r^{-2}$ for a 
    wind-like medium.}
  \tablenotetext{b}{We are only able to calculate an upper limit for the host 
    extinction in this case.}
\label{tab:050820A}
\end{deluxetable}



==> tab4.tex <==
\ProvidesFile{060418models.tab.tex}

\begin{deluxetable}{r|cccccccc}
  \tabletypesize{\scriptsize}
  \tablecaption{GRB\,060418 Forward Shock Best Fit Parameters}
  \tablecolumns{9}
  \tablewidth{0pc}
  \tablehead{\colhead{Medium Type\tablenotemark{a}} & \colhead{$E_{\mathrm{KE,iso}}$} & 
             \colhead{$n$ / $A_{*}$\tablenotemark{b}} & \colhead{$\epsilon_{e}$} &
             \colhead{$\epsilon_{B}$} & \colhead{$\theta$} & \colhead{$p$} &
             \colhead{$A_{V}$(host)} & \colhead{$\chi^{2}_{\mathrm{r}}$ 
             (d.o.f.)} \\ & \colhead{($10^{52}$\,erg)} & \colhead{(cm$^{-3}$ / g cm$^{-1}$)} &
             & \colhead{($\%$)} & \colhead{($^{\circ}$)} & & \colhead{(mag)} &
            }
  \startdata
  ISM & $3.2_{-0.6}^{+1.2}$ & $0.18_{-0.06}^{+0.08}$ & 
     $0.33$\tablenotemark{c} & $31_{-1}^{+2}$ & $13.9_{-1.6}^{+2.1}$ & 
     $2.06 \pm 0.01$ & $0.08 \pm 0.03$ & 1.15 (82) \\
  Wind & $0.12_{-0.01}^{+0.03} $ & $0.35 \pm 0.12$ &
     $0.06_{-0.02}^{+0.01}$ & $15_{-1}^{+14}$ & $22.5_{-2.5}^{+0.9}$ & 
     $1.97_{-0.04}^{+0.02}$ & $< 10^{-4}$\tablenotemark{d} & 1.10 (81) \\
  \enddata
  \tablenotetext{a}{Radial profile of the circumburst medium.  $\rho \propto 
    r^{0}$ for an ISM-like medium; $\rho \propto r^{-2}$ for a wind-like medium.}
  \tablenotetext{b}{For a wind-like medium, the density parameter is better
    known as $A_{*}$, where $\rho \equiv 5 \times 10^{11} A_{*} r^{-2}$.}
  \tablenotetext{c}{The best fit was achieved with $\epsilon_{e}$ fixed to its equipartition
    value.}
  \tablenotetext{d}{We could only calculate an upper limit for the host
     extinction.}
\label{tab:060418}
\end{deluxetable}



==> tab5.tex <==
\ProvidesFile{080319Bmodels.tab.tex}

\begin{deluxetable}{r|cccccccc}
  \tabletypesize{\scriptsize}
  \tablecaption{GRB\,080319B Forward Shock Best Fit Parameters}
  \tablecolumns{9}
  \tablewidth{0pc}
  \tablehead{\colhead{Medium Type\tablenotemark{a}} & 
             \colhead{$E_{\mathrm{KE,iso}}$} & \colhead{$A_{*}$} & 
             \colhead{$\epsilon_{e}$} & \colhead{$\epsilon_{B}$} & 
             \colhead{$\theta$} & \colhead{$p$} & \colhead{$A_{V}$(host)} & 
             \colhead{$\chi^{2}_{\mathrm{r}}$ (d.o.f.)} \\ 
             & \colhead{($10^{52}$\,erg)} & \colhead{(cm$^{-3}$ / g cm$^{-1}$)} &
             & \colhead{($\%$)} & \colhead{($^{\circ}$)} & & \colhead{(mag)} &
            }
  \startdata
  Wind-1 & $8.0_{-0.5}^{+0.8}$ & $0.0056_{-0.0003}^{+0.0004}$ & 
     $0.11 \pm 0.01$ & $33$\tablenotemark{c} & $3.6 \pm 0.2$ & 
     $2.10 \pm 0.02$ & $< 0.04$\tablenotemark{d} & 1.13 (157) \\
  Wind-2 & $4.9_{-0.1}^{+3.2} $ & $0.015 \pm 0.005$ &
     $0.0099_{-0.0001}^{+0.005}$ & $33$\tablenotemark{c} & $7.0_{-0.1}^{+0.7}$ & 
     $1.85 \pm 0.02$ & $0.07_{-0.02}^{+0.04}$ & 1.12 (157) \\
  \enddata
  \tablenotetext{a}{Radial profile of the circumburst medium.  $\rho 
    \propto r^{0}$ for an ISM-like medium; $\rho \propto r^{-2}$ for a wind-like 
    medium.}
  \tablenotetext{b}{For a wind-like medium, the density parameter is better
    known as $A_{*}$, where $\rho \equiv 5 \times 10^{11} A_{*} r^{-2}$.}
  \tablenotetext{c}{The best fit was achieved with $\epsilon_{B}$ fixed to 
    its equipartition value.}
  \tablenotetext{d}{We could only calculate an upper limit for the host
     extinction.}
\label{tab:080319B}
\end{deluxetable}



==> tab6.tex <==
\ProvidesFile{energy.tab.tex}

\begin{deluxetable}{r|cccccccc}
  \tabletypesize{\scriptsize}
  \tablecaption{Collimation and Energetics of \Swift\ GRBs}
  \tablecolumns{5}
  \tablewidth{0pc}
  \tablehead{\colhead{GRB} & \colhead{$t_{\mathrm{jet}}$} & \colhead{$\theta$} &
    \colhead{$E_{\gamma}$} & \colhead{$E_{\mathrm{KE}}$} \\ & \colhead{(d)} &
    \colhead{($^{\circ}$)} & \colhead{($10^{51}$\,erg)} & \colhead{($10^{51}$\,erg)}
    }
  \startdata
  050820A & $11.1_{-1.7}^{+0.1}$ & $3.0 \pm 0.1$ & $6.5_{-1.5}^{+3.2}$ &
    $36.1_{-9.4}^{+11.3}$ \\ 
  050904 & $2.6 \pm 1.0$ & 8.0 & $12.9_{-3.9}^{+6.6}$ & $8.6_{-4.3}^{+8.4}$ \\ 
  060418 & $7.6_{-2.2}^{+2.0}$ & $22.5_{-2.5}^{+0.9}$ & $3.0_{-1.1}^{+3.8}$ & 
    $0.94_{-0.35}^{+0.22}$ \\
  070125 & $3.69_{-0.07}^{+0.03}$ & $13.2 \pm 0.6$ & $25.3_{-4.6}^{+5.1}$ &
    $1.7_{-0.2}^{+0.4}$ \\
  080319B & $11.8_{-1.3}^{+0.8}$ & $7.0_{-0.1}^{+0.7}$ & $10.2_{-0.1}^{+3.2}$ &
    $0.35_{-0.01}^{+0.38}$ \\
  \enddata
\label{tab:energy}
\end{deluxetable}



==> tab7.tex <==
\ProvidesFile{060418opt.tab.tex}

\begin{deluxetable}{crrrrr}
  \tabletypesize{\scriptsize}
  \tablecaption{Optical/NIR Observations of GRB\,060418}
  \tablecolumns{7}
  \tablewidth{0pc}
  \tablehead{\colhead{UT Date\tablenotemark{a}} & 
             \colhead{Telescope / Instrument} & \colhead{Time Since 
             Burst\tablenotemark{b}} & \colhead{Filter} &
             \colhead{Exposure Time} & \colhead{Magnitude\tablenotemark{c}} \\
             & & \colhead{(s)} & & \colhead{(s)} &
            }
  \startdata
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    2006 Apr 18.2261 & PAIRITEL & $1.161 \times 10^{4}$ & \J & 4206.5 &
     $17.11 \pm 0.06$ \\
    2006 Apr 18.2261 & PAIRITEL & $1.161 \times 10^{4}$ & \Hm & 4206.5 &
     $16.17 \pm 0.10$ \\
    2006 Apr 18.2261 & PAIRITEL & $1.161 \times 10^{4}$ & \Ks & 4206.5 &
     $15.43 \pm 0.11$ \\
    2006 Apr 18.2429 & P60 & $1.011 \times 10^{4}$ & \Rc & 600.0 & 
     $18.60 \pm 0.06$ \\
    2006 Apr 18.2511 & P60 & $1.083 \times 10^{4}$ & \ip & 600.0 & 
     $18.57 \pm 0.07$ \\
    2006 Apr 18.2593 & P60 & $1.153 \times 10^{4}$ & \Vc & 600.0 & 
     $19.36 \pm 0.09$ \\
    2006 Apr 18.2675 & P60 & $1.224 \times 10^{4}$ & \Rc & 600.0 & 
     $18.83 \pm 0.06$ \\
    2006 Apr 18.2757 & P60 & $1.296 \times 10^{4}$ & \ip & 600.0 & 
     $18.80 \pm 0.08$ \\
    2006 Apr 18.2841 & P60 & $1.368 \times 10^{4}$ & \Vc & 600.0 & 
     $19.50 \pm 0.13$ \\
    2006 Apr 18.2924 & P60 & $1.440 \times 10^{4}$ & \Rc & 600.0 & 
     $19.03 \pm 0.09$ \\
    2006 Apr 18.3009 & P60 & $1.513 \times 10^{4}$ & \ip & 600.0 & 
     $19.06 \pm 0.09$ \\
    2006 Apr 18.3021 & PAIRITEL & $1.545 \times 10^{4}$ & \J & 682.8 &
     $17.57 \pm 0.08$ \\
    2006 Apr 18.3021 & PAIRITEL & $1.545 \times 10^{4}$ & \Hm & 682.8 &
     $16.39 \pm 0.09$ \\
    2006 Apr 18.3021 & PAIRITEL & $1.545 \times 10^{4}$ & \Ks & 682.8 &
     $16.19 \pm 0.14$ \\
    2006 Apr 18.3098 & P60 & $1.590 \times 10^{4}$ & \Vc & 600.0 & 
     $19.61 \pm 0.20$ \\
    2006 Apr 18.3151 & PAIRITEL & $1.781 \times 10^{4}$ & \J & 2283.8 &
     $17.55 \pm 0.06$ \\
    2006 Apr 18.3151 & PAIRITEL & $1.781 \times 10^{4}$ & \Hm & 2283.8 &
     $16.70 \pm 0.09$ \\
    2006 Apr 18.3151 & PAIRITEL & $1.781 \times 10^{4}$ & \Ks & 2283.8 &
     $16.32 \pm 0.12$ \\
    2006 Apr 18.3271 & P60 & $1.740 \times 10^{4}$ & \Rc & 600.0 & 
     $19.38 \pm 0.10$ \\
    2006 Apr 18.3376 & P60 & $1.830 \times 10^{4}$ & \ip & 600.0 & 
     $19.38 \pm 0.09$ \\
    2006 Apr 18.3465 & P60 & $1.907 \times 10^{4}$ & \Vc & 600.0 & 
     $19.96 \pm 0.15$ \\
    2006 Apr 18.3553 & P60 & $1.983 \times 10^{4}$ & \Rc & 600.0 & 
     $19.55 \pm 0.11$ \\
    2006 Apr 18.3567 & PAIRITEL & $2.140 \times 10^{4}$ & \J & 2283.8 &
     $17.91 \pm 0.08$ \\
    2006 Apr 18.3567 & PAIRITEL & $2.140 \times 10^{4}$ & \Hm & 2283.8 &
     $17.03 \pm 0.09$ \\
    2006 Apr 18.3567 & PAIRITEL & $2.140 \times 10^{4}$ & \Ks & 2283.8 &
     $16.50 \pm 0.20$ \\
    2006 Apr 18.3642 & P60 & $2.059 \times 10^{4}$ & \ip & 600.0 & 
     $19.52 \pm 0.13$ \\
    2006 Apr 18.3837 & P60 & $2.258 \times 10^{4}$ & \Vc & 1200.0 & 
     $20.36 \pm 0.15$ \\
    2006 Apr 18.3917 & P60 & $2.297 \times 10^{4}$ & \ip & 600.0 & 
     $19.61 \pm 0.08$ \\
    2006 Apr 18.3935 & P60 & $2.343 \times 10^{4}$ & \Rc & 1200.0 & 
     $19.78 \pm 0.09$ \\
    2006 Apr 18.3983 & PAIRITEL & $2.501 \times 10^{4}$ & \J & 2307.3 &
     $18.17 \pm 0.08$ \\
    2006 Apr 18.3983 & PAIRITEL & $2.501 \times 10^{4}$ & \Hm & 2307.3 &
     $17.23 \pm 0.12$ \\
    2006 Apr 18.3983 & PAIRITEL & $2.501 \times 10^{4}$ & \Ks & 2307.3 &
     $16.58 \pm 0.15$ \\
    2006 Apr 18.4222 & P60 & $2.561 \times 10^{4}$ & \ip & 600.0 & 
     $19.90 \pm 0.11$ \\
    2006 Apr 18.4403 & PAIRITEL & $2.862 \times 10^{4}$ & \J & 2283.8 &
     $18.38 \pm 0.10$ \\
    2006 Apr 18.4403 & PAIRITEL & $2.862 \times 10^{4}$ & \Hm & 2283.8 &
     $17.57 \pm 0.13$ \\
    2006 Apr 18.4403 & PAIRITEL & $2.862 \times 10^{4}$ & \Ks & 2283.8 &
     $16.39 \pm 0.11$ \\
    2006 Apr 18.4408 & P60 & $2.722 \times 10^{4}$ & \Rc & 600.0 & 
     $20.31 \pm 0.16$ \\
    2006 Apr 18.4456 & P60 & $2.793 \times 10^{4}$ & \Vc & 1200.0 & 
     $20.87 \pm 0.23$ \\
    2006 Apr 18.4544 & P60 & $2.839 \times 10^{4}$ & \ip & 600.0 & 
     $19.96 \pm 0.12$ \\
    2006 Apr 18.4552 & P60 & $2.877 \times 10^{4}$ & \Rc & 1200.0 & 
     $20.09 \pm 0.12$ \\
    2006 Apr 18.4818 & PAIRITEL & $3.174 \times 10^{4}$ & \J & 1672.6 &
     $18.52 \pm 0.11$ \\
    2006 Apr 18.4818 & PAIRITEL & $3.174 \times 10^{4}$ & \Hm & 1672.6 &
     $17.94 \pm 0.18$ \\
    2006 Apr 18.4818 & PAIRITEL & $3.174 \times 10^{4}$ & \Ks & 1672.6 &
     $17.22 \pm 0.18$ \\
    2006 Apr 18.4864 & P60 & $3.116 \times 10^{4}$ & \ip & 600.0 & 
     $20.02 \pm 0.13$ \\
    2006 Apr 19.3560 & P60 & $1.072 \times 10^{5}$ & \Rc & 1800.0 & 
     $> 21.02$ \\
    2006 Apr 19.3581 & PAIRITEL & $1.079 \times 10^{5}$ & \J & 2283.8 &
     $> 19.06$ \\
    2006 Apr 19.3581 & PAIRITEL & $1.079 \times 10^{5}$ & \Hm & 2283.8 &
     $> 18.61$ \\
    2006 Apr 19.3581 & PAIRITEL & $1.079 \times 10^{5}$ & \Ks & 2283.8 &
     $> 17.89$ \\
    2006 Apr 19.3669 & P60 & $1.081 \times 10^{5}$ & \ip & 1800.0 & 
     $> 21.49$ \\
    2006 Apr 19.3782 & P60 & $1.091 \times 10^{5}$ & \Vc & 1800.0 & 
     $> 21.36 $ \\
    2006 Apr 20.3405 & P60 & $1.920 \times 10^{5}$ & \Rc & 1800.0 & 
     $> 21.75$ \\
    2006 Apr 20.3535 & P60 & $1.931 \times 10^{5}$ & \ip & 1800.0 & 
     $> 22.19$ \\
    2006 Apr 19.2870 & P200 / LFC & $1.002 \times 10^{5}$ & \rp & 
     300.0 & $22.07 \pm 0.10$ \\
    2006 Apr 19.2954 & P200 / LFC & $1.009 \times 10^{5}$ & \ip & 
     300.0 & $21.73 \pm 0.10$ \\
    2006 Apr 19.3033 & P200 / LFC & $1.016 \times 10^{5}$ & \zp & 
     300.0 & $21.52 \pm 0.29$ \\
    2006 Apr 19.3122 & P200 / LFC & $1.024 \times 10^{5}$ & \gp & 
     300.0 & $22.75 \pm 0.15$ \\
    2006 Apr 22.5584 & Keck / LRIS & $3.833 \times 10^{5}$ & \Rc &
     1200.0 & $23.31 \pm 0.08$ \\
    2006 Apr 22.5590 & Keck / LRIS & $3.835 \times 10^{5}$ & \gp &
     1500.0 & $> 23.08$ \\
    2006 May 9.4161 & \hst\ / ACS & $1.839 \times 10^{6}$ & {\it F625W} & 
     4220.0 & $27.06 \pm 0.15$ \\
    2006 May 9.6130 & \hst\ / ACS & $1.856 \times 10^{6}$ & {\it F775W} & 
     4220.0 & $26.96 \pm 0.19$ \\
    2006 May 20.2953 & \hst\ / ACS & $2.779 \times 10^{6}$ & {\it F625W} & 
     5500.0 & $> 27.53$ \\
    2006 May 20.4926 & \hst\ / ACS & $2.796 \times 10^{6}$ & {\it F775W} & 
     3700.0 & $> 26.93$ \\
    2006 Jun 1.7528 & \hst\ / ACS & $3.855 \times 10^{6}$ & {\it F625W} & 
     8772.0 & $> 28.04$ \\
    2006 Jun 2.0193 & \hst\ / ACS & $3.879 \times 10^{6}$ & {\it F775W} & 
     8772.0 & $> 27.51$ \\
    2006 Jul 11.1211 & \hst\ / ACS & $7.343 \times 10^{6}$ & {\it F625W} & 
     8772.0 & $> 28.16$ \\
    2006 Jul 12.5207 & \hst\ / ACS & $7.378 \times 10^{6}$ & {\it F775W} & 
     8772.0 & $> 28.10$ \\
    2006 Jul 13.1036 & \hst\ / ACS & $7.428 \times 10^{6}$ & {\it F555W} &
     4386.0 & $> 27.53$ \\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \enddata
  \tablenotetext{a}{UT at beginning of exposure.}
  \tablenotetext{b}{Time from midpoint of exposure to \Swift-BAT trigger.}
  \tablenotetext{c}{Reported magnitudes have not been corrected for Galactic
    extinction ($E(B-V)= 0.22$\,mag; \citealt{sfd98}).  Observations in the
    \Vc,\Rc, \J, \Hm, and \Ks\ filters are referenced to Vega, while all other 
    filters use the AB magnitude system \citep{og83}.}
\label{tab:060418opt}
\end{deluxetable}


